Heavy quark pair production in gluon fusion at next-to-next-to-leading ${\cal O}(\alpha_s^4)$ order: One-loop squared contributions

We calculate the next-to-next-to-leading order ${\cal O}(\alpha_s^4)$ one-loop squared corrections to the production of heavy-quark pairs in the gluon-gluon fusion process. Together with the previously derived results on the $q \bar{q}$ production channel the results of this paper complete the calculation of the one-loop squared contributions of the next-to-next-to-leading order ${\cal O}(\alpha_s^4)$ radiative QCD corrections to the hadroproduction of heavy flavors. Our results, with the full mass dependence retained, are presented in a closed and very compact form, in dimensional regularization.

==> nlo <==
%auto-ignore
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%   notations   %%%%%%%%%%%%%%%%%%%%%
%
%
%    Heavy quark pair production in gluon fusion at next-to-next-to-leading
%       ${\cal O}(\alpha_s^4)$ order: The one-loop squared contributions
%
%
%   This file in REDUCE format gives coefficients in Appendix A
%
%                       Definitions:
%  ep = \epsilon 
%  nc = 3, cf = 4/3, da=8 - color factors defined in the paper;
%
%  bet^2=1-4*m^2/s, z2=s+2*t, z2u=s+2*u, zt=2*m^2+t, zu=2*m^2+u;
%  den=D=m^2*s-t*u, tt=t+m^2, uu=u+m^2; 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%   Appendix A, Eq.(A2)

b12:= 16*Den/s/bet^2$
b15:= - b12$
c11:= 4*( 8*m^4 - z2^2/s*(2*m^2 - s + 2*m^2/bet^2) )$
c12:= 8*t/s*(4*m^2*zt + 2*s*t + t^2)$
c12u:= 8*u/s*(4*m^2*zu + 2*s*u + u^2)$
c13:= 8*t/s*(4*m^2*zt + t*z2)$
c13u:= 8*u/s*(4*m^2*zu + u*z2u)$
c14:= 4*(4*m^2*s + 3*s^2 - 8*t*u)$
c15:= 4*(8*m^4 - 3*s^2 + 2*t*u)$
c16:= - 4*bet^2*(2*m^2*s + s^2 + 2*t*u)$
d11:= 4*( 2*m^2*(2*Den + s*zt*bet^2 - t^2*bet^2) + s^2*t*bet^2 + t^3 )$
d11u:= 4*( 2*m^2*(2*Den + s*zu*bet^2 - u^2*bet^2) + s^2*u*bet^2 + u^3 )$
d12:= 4*(8*m^2*Den - s*t*u*bet^2 + 2*t^2/s*(t^2 + u^2))$
d12u:= 4*(8*m^2*Den - s*t*u*bet^2 + 2*u^2/s*(t^2 + u^2))$
d13:= 8*(8*m^2*Den - 8*m^4*t*u/s - s*t*u*bet^2 + 2*t^2*u^2/s)$

v1 :=     b2(0)*b12 + b5(0)*b15 
        + c1(0)*c11 + c2(0)*c12 + c2u(0)*c12u + c3(0)*c13 + c3u(0)*c13u
        + c4(0)*c14 + c5(0)*c15 + c6(0)*c16
        + d1(0)*d11 + d1u(0)*d11u + d2(0)*d12 + d2u(0)*d12u + d3(0)*d13$

%%%%%%%%%%%%%   Appendix A, Eq.(A3)

b12:=4*(2*s - z2^2/s/bet^2 )$
b15:=-b12$
c11:=2*( bet^2*(s^3*(8*m^2 + s) - 8*t^2*u^2)/Den
                                         + 16*m^2/s*(s^2 + t*u + Den/bet^2) )$
c12:= - 4*t^2*(10 - t/s*(2*t*u*bet^2 + 2*s^2 - 3*t^2)/Den)$
c12u:= - 4*u^2*(10 - u/s*(2*t*u*bet^2 + 2*s^2 - 3*u^2)/Den)$
c13:= - 4*t^2*(6 - t/s*(2*t*u*bet^2 + 2*s^2 - 4*s*t - 5*t^2)/Den)$
c13u:= - 4*u^2*(6 - u/s*(2*t*u*bet^2 + 2*s^2 - 4*s*u - 5*u^2)/Den)$
c14:= - 2*( s^3*(2*m^2 - s) - 8*t*u*(m^2*s + t^2 + u^2) )/Den$
c15:= 2*( bet^2*(s^3*(6*m^2 - s) + 4*t^2*u^2)/Den + 8*s^2 - 12*m^4*z2^2/Den )$
c16:= 2*( bet^2*(s^3*(8*m^2 - s) - 4*t^2*u^2)/Den + 8*m^2*s - 4*m^4*z2^2/Den )$
d11:= - 2*t*( 2*s^2*bet^2 - s^2*t*bet^2*(2*m^2*z2^2/s^2 + 4*m^2 + t)/Den 
                                                           + 2*t*zt + 2*s^2 )$
d11u:= - 2*u*( 2*s^2*bet^2 - s^2*u*bet^2*(2*m^2*z2u^2/s^2 + 4*m^2 + u)/Den 
                                                           + 2*u*zu + 2*s^2 )$
d12:= - 2*t*( 2*s*(s - u) + t^2*(s^2 + 8*t*u - 8*u^3/s)/Den )$
d12u:= - 2*u*( 2*s*(s - t) + u^2*(s^2 + 8*t*u - 8*t^3/s)/Den )$
d13:= 4*t*u*( 4*s - t^2*u^2/s^2*(8*m^2 - 7*s)/Den )$

v1ep := ep*(
          b2(0)*b12 + b5(0)*b15
        + c1(0)*c11 + c2(0)*c12 + c2u(0)*c12u + c3(0)*c13 + c3u(0)*c13u
        + c4(0)*c14 + c5(0)*c15 + c6(0)*c16 
        + d1(0)*d11 + d1u(0)*d11u + d2(0)*d12 + d2u(0)*d12u + d3(0)*d13 )$

%%%%%%%%%%%%%%%%%   Appendix A, Eq.(A4)

c11:= 8*s*(s - 2*m^2*z2^2/Den)$
c12:= - 8*t^2*(3*u/s + t*(m^2 - u)/Den)$
c12u:= - 8*u^2*(3*t/s + u*(m^2 - t)/Den)$
c13:= 8*t^2*(2 + t*u*(1 - 3*t/s)/Den)$
c13u:= 8*u^2*(2 + t*u*(1 - 3*u/s)/Den)$
c14:= - 16*s^2*t*u/Den$
c15:= - 4*s*(s + 2*m^2*z2^2/Den)$
c16:= 4*s*(s - 2*m^2*z2^2/Den)$
d11:= - 4*s*t*( 2*m^2 - s + t*(bet^2*t*u + m^2*z2^2/s)/Den )$
d11u:= - 4*s*u*( 2*m^2 - s + u*(bet^2*t*u + m^2*z2u^2/s)/Den )$
d12:= 4*s*t*(s - 4*t^2*u/Den)$
d12u:= 4*s*u*(s - 4*t*u^2/Den)$
d13:= - 8*t*u*(s + 3*t^2*u^2/s/Den)$

v1ep2 := ep^2*(
          c1(0)*c11 + c2(0)*c12 + c2u(0)*c12u + c3(0)*c13 + c3u(0)*c13u
        + c4(0)*c14 + c5(0)*c15 + c6(0)*c16
        + d1(0)*d11 + d1u(0)*d11u + d2(0)*d12 + d2u(0)*d12u + d3(0)*d13 )$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   Appendix A, Eq.(A5)

con2:= - 16/3*z2/s*( m^2*(nlf + 1) + (2*cf - nc)*3*Den/s/bet^2
                           - nc*(m^2 + Den*6*(10*m^2 - s)/s^2/bet^4) )$
b22:= - 8*z2/s^2*( 8*m^4 - (2*cf - nc)*Den*(2 + 1/bet^2) )$
b25:= - nc*8*z2*( Den*(16*m^2 - s)/s/bet^4 + t*u )/s^2$
c21:= - nc*16*m^2*Den*z2*(8*m^2 + s)/s^3/bet^4$
c24:= nc*4*z2*(Den - 2*t*u)/s$
c25:= - 32*m^4*z2/s$
c26:= - (2*cf - nc)*16*Den*z2*(2*m^2 - s)/s^2$

v2 := con2 + b2(0)*b22 + b5(0)*b25 + c1(0)*c21 + c4(0)*c24 + c5(0)*c25 + c6(0)*c26$

%%%%%%%%%%%%%%%%   Appendix A, Eq.(A6)

con2:= 16/3*z2*( t*u*(nlf + 1) + (2*cf - nc)*3*Den/bet^2
                    - nc*(36*m^2*Den/(s*bet^4) - t*u*(4*m^2 - 7*s)/(s*bet^2)) )/s^2$
b22:= 8*z2*( 8*m^2*t*u/s + (2*cf - nc)*(2*t*u - Den/bet^2) )/s^2$
b25:= - nc*8*z2*( 2*(Den + 2*m^2*t*u/s)/bet^2 - 3*m^2*z2^2/(s*bet^4) )/s^2$
c21:= nc*16*m^2*z2*(3*Den/bet^4 + 2*t*u/bet^2)/s^2$
c24:= nc*12*t*u*z2/s$
c25:= 32*m^2*t*u*z2/s^2$
c26:= - (2*cf - nc)*16*t*u*z2*(2*m^2 - s)/s^2$

v2ep := ep*( con2 + b2(0)*b22 + b5(0)*b25 
             + c1(0)*c21 + c4(0)*c24 + c5(0)c25 + c6(0)*c26 )$

%%%%%%%%%%%%%%%%%%%%

v2ep2 := 0$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    Appendix A, Eq.(A7)
con3:= 16/TT*( cf*( Den*bet^2*(8*m^2*TT/t^2 + 2)
                    - Den*(6*zt/t - 2 - t/s)
                    + 2*m^2*(4*zt*(m^2/s - 1) - m^2)
                    - Den*(1 + 4*t/s)/bet^2 )
             -   nc*( Den*2*m^2/s/t^2*(2*Den + t*u)
                    - 2*m^2*t*u/s
                    - Den*4*m^2*(s + 4*t)/(s^2*bet^2) ) )$
b31:= 16*( cf*( 2*m^2*bet^2*(TT - 2*s - Den*(2*TT + t)/t^2)
                       + Den*(3*zt/t + t/s) - 2*m^2*u*(2 + 5*t/s) )/TT
         + nc*2*Den*(Den/s - t)/t^2 )$
b32:= (2*cf - nc)*16*Den/(s*bet^2)$
b35:= nc*8*( - 8*m^2*Den/(s^2*bet^2) - t*bet^2 + t^2*z2/s^2 )$
c31:= nc*8*( t^3 + u^3 - 4*t^2*TT - s*Den/bet^2 - s^2*bet^2*(m^2 - t) )/s$
c32:= - (2*cf - nc)*16*( 2*m^2*z2*(m^2*s/t - zt) + t*(s^2 + t^2) )/s$
c33:= nc*16*t*( 4*Den/s - t*bet^2 + s )$
c34:= nc*4*( - s^2*bet^2 + 3*z2*(m^2*s - t^2)/s - 3*s*u + 2*t^2 )$
c35:= (2*cf - nc)*8*(2*TT*(2*m^2 + s) - u^2)$
c36:= - (2*cf - nc)*8*(4*m^2*Den/s - 4*m^2*t*bet^2 + 3*t*zt - z2^2)$
d31:= - (2*cf - nc)*8*( m^2*s^2*bet^4 - 2*m^2*t*bet^2*(s - t)
                                                      + s*t^2*bet^2 - t^3 - s*Den )$
d32:= nc*8*(8*m^2*Den - s*t*u*bet^2 + 2*t^2*(t^2 + u^2)/s)$


v3 := ( con3 + b1(0)*b31 + b2(0)*b32 + b5(0)*b35
      + c1(0)*c31 + c2(0)*c32 + c3(0)*c33 + c4(0)*c34 + c5(0)*c35 + c6(0)*c36
      + d1(0)*d31 + d2(0)*d32 )$


%%%%%%%%%%%%%%%%%%   Appendix A, Eq.(A8)

con3:= 16*( cf*( Den*(16*m^2*Den/(s*t^2) - 24*m^4/t^2 + 4 - t/s + 2*t/(s*bet^2))
                        + 2*m^2*(4*m^2 - 6*t - 9*t^2/s)
                        + 4*m^2*t^2*z2/(s^2*bet^2) )/TT
                 + nc*2*( 2*m^4*s/t^2 + t + Den*z2/(s*t)
                        - Den*(4*m^2 + 3*s)/(s^2*bet^2) + t*z2/(s*bet^2) ) )$
b31:= 16*(cf*(4*m^4*Den/t^2 - 6*TT*Den/t - 2*m^2*Den/s - t*Den/s - 5*m^2*zt + t^2)
                    - nc*(2*m^2*Den^2/s/t^2 + 2*t*Den/s - m^4 + t^2))/TT$
b32:= - (2*cf - nc)*8*t*(2 + z2/(s*bet^2))$
b35:= nc*8*(2*Den/bet^2 + 6*m^2*z2/bet^2 - 3*t^2 - 2*t^3/s)/s$
c31:= - nc*4*( 2*m^2*z2^2/s - 4*s^2 - 4*t^2 - 4*m^2*(4*zt + t*z2/s)/bet^2
               + 2*t*u*zt*(4*s + 3*t^2/s + u^2/s)/Den + s*t^2*(2*t*bet^2 - z2)/Den )$
c32:= (2*cf - nc)*8*( bet^2*t*(6*s*Den - 4*m^2*t*u - s*t^2)
                              + Den*2*(2*m^4*s/t - s*zt + Den*t/s - t^2)
                              - 4*m^2*t^3*z2/s )/Den$
c33:= - nc*8*t^2*(4*s/t + 14 - s*t*(4*bet^2 - 8*t*TT/s^2 + 5)/Den)$
c34:= - nc*4*(2*s^2 + 2*t^3/s - 2*s*u + m^2*s*t*(9*s + 7*t)/Den - t^4*(9 + 8*t/s)/Den)$
c35:= - (2*cf - nc)*4*(2*m^2*z2^2/s - 2*t^2 - 4*s*bet^2*(s - m^2*t*u/Den)
                                                          + t^2*(8*m^2*t + s^2)/Den)$
c36:= - (2*cf - nc)*4*s*t*(7*bet^2 + 2*u^2*bet^2/(s*t) + 2*s/t + 5
                                         + bet^2*(2*m^2*z2^2/s - 3*s*t - 4*t^2)/Den)$
d31:= - (2*cf - nc)*4*s*t^2*(2*s*bet^2/t + 2*s/t + 2*t/s + 4*m^4*z2^2/(s^2*Den) 
                                          - bet^2*(6*m^2*s - 4*m^2*t*u/s + s*t)/Den)$
d32:= - nc*4*t*(4*s^2 + 2*s*t + t^2*(z2^2 + 12*t*u - 8*u^3/s)/Den)$


v3ep := ep*( con3 + b1(0)*b31 + b2(0)*b32 + b5(0)*b35
        + c1(0)*c31 + c2(0)*c32 + c3(0)*c33 + c4(0)*c34 + c5(0)*c35 + c6(0)*c36
        + d1(0)*d31 + d2(0)*d32 )$

%%%%%%%%%%%%%%%%%   Appendix A, Eq.(A9)

con3:=  - 16*( cf*( 2*m^2*(6*Den/t + 4*m^2 + t)
                           - 4*m^2*(3*Den + t*z2)/(s*bet^2) + Den/bet^2 )/TT
                      - nc*2*(u - 4*m^2*zu/(s*bet^2)) )$
b31:= 16*( cf*zt*(3*Den/t + 2*m^2)/TT - nc*2*m^2 )$
b32:= - (2*cf - nc)*32*m^2*z2/(s*bet^2)$
b35:= - nc*64*m^2*z2/(s*bet^2)$
c31:= - nc*8*s*(4*t + 2*m^2*t*(s + 4*t + z2^2/(s*bet^2))/Den + s/bet^2 )$
c32:= (2*cf - nc)*16*( 2*m^2*s + t*u + 2*m^2*t*(m^2*s - t^2)/Den )$
c33:= nc*16*t*(s + 2*t*(m^2*s + t*u)/Den)$
c34:= nc*8*s*(s + 2*t*(m^2*s + t*u)/Den)$
c35:= (2*cf - nc)*8*s*(u - 2*m^2*t*z2/Den )$
c36:= - (2*cf - nc)*8*( 2*m^2*z2*(m^2*s - t^2)/Den + s*u )$
d31:= - (2*cf - nc)*8*t*(s*zu + 2*m^2*t*z2^2/Den)$
d32:= nc*8*s*t*(s - 4*t^2*u/Den)$

v3ep2 := ep^2*( con3 + b1(0)*b31 + b2(0)*b32 + b5(0)*b35
        + c1(0)*c31 + c2(0)*c32 + c3(0)*c33 + c4(0)*c34 + c5(0)*c35 + c6(0)*c36
        + d1(0)*d31 + d2(0)*d32 )$



END;


==> nloep2f <==
%auto-ignore
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%   notations   %%%%%%%%%%%%%%%%%%%%%
%
%
%    Heavy quark pair production in gluon fusion at next-to-next-to-leading
%       ${\cal O}(\alpha_s^4)$ order: The one-loop squared contributions
%
%
%   This file in REDUCE format gives coefficients in Appendix C
%
%                       Definitions:
%  ep = \epsilon
%  nc = 3, cf = 4/3, da=8 - color factors defined in the paper;
%
%  bet^2=1-4*m^2/s, z2=s+2*t, z2u=s+2*u, zt=2*m^2+t, zu=2*m^2+u;
%  den=D=m^2*s-t*u, tt=t+m^2, uu=u+m^2;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%   Appendix C, Eq.(C1)

cc1:= -s*bet^2*(18*m^2*s^2 - s^3 + 2*(2*m^2 + s)*z2^2) - Den*8*m^2*s$
cc6:= -s*bet^2*z2^2 + 16*s*Den + 6*s*t*u$


%%%%%%%%%%%   Appendix C, Eq.(C2)

c11:= - s*cc1/(t*u*Den)$
c12:= 2*t*( cc6*t/s + 2*m^2*s*u - s^2*zt + t^3 )/(u*Den)$
c12u:= 2*u*( cc6*u/s + 2*m^2*s*t - s^2*zu + u^3 )/(t*Den)$
c13:= 2*t^2*( cc6/s + 2*s^2 + u^2 )/(u*Den)$
c13u:= 2*u^2*( cc6/s +  2*s^2 + t^2 )/(t*Den)$
c14:= s^2*( cc6 + 2*s*(u^2 - s*t) )/(t*u*Den)$
c15:= - s*( cc1 - 2*s^2*(2*Den - t*u*bet^2 - z2^2) )/(t*u*Den)$
c16:= s^2*bet^2*cc6/(t*u*Den)$
d11:= s*t*bet^2*( cc6 - s*u*z2 )/(u*Den)$
d11u:= s*u*bet^2*( cc6 - s*t*z2u )/(t*Den)$
d12:= s*t*( cc6 + s^3 - s^2*t )/(u*Den)$
d12u:= s*u*( cc6 + s^3 - s^2*u )/(t*Den)$
d13:= 2*t*u*( cc6/s - s*t + u^2 )/Den$

eps2ep2del:= ( c1(0)*c11 + c2(0)*c12 + c2u(0)*c12u + c3(0)*c13 + c3u(0)*c13u
             + c4(0)*c14 + c5(0)*c15 + c6(0)*c16
             + d1(0)*d11 + d1u(0)*d11u + d2(0)*d12 + d2u(0)*d12u + d3(0)*d13)$


%%%%%%%%%%%   Appendix C, Eq.(C3)

colfac:= - (cf + nc/2*t/s)$


tno0:=8*z2*
  ( 4/3*s*(nlf + 1) + b2(0)*(16*m^2 + 5*s) + b5(0)*5*s*nlf + c5(0)*18*m^2*s)/(9*s^2)$

eps2ep2no:= - tno0*m^2*s/t/u$


%%%%%%%%%%%   Appendix C, Eq.(C4)

con2:= 32*( 2*m^2*(2*m^2*u^2/t^2 - s^2/t + 2*t - 8*Den*TT/t^2)
                  - s*bet^2*(2*Den/t + m^2) + Den*4*UU/(s*bet^2) )/(t*u)$
c22:= 2*zt/(s*bet^2)*c26$
c25:= zt/(t*bet^2)*c26$
c26:= 4*s*bet^2*( cc6/u - s*z2 )/Den$
d21:= - t*c26$

eps2ep2cf:= cf*(con2 + c2(0)*c22 + c5(0)*c25 + c6(0)*c26 + d1(0)*d21)$


%%%%%%%%%%%   Appendix C, Eq.(C5)

con3:= - 16*m^2*( 18*s^2*zt/t^2 + 82/3*s + 2/3*t
                  - 9*s*z2/(s*bet^2) + Den*144*zu/(s^2*bet^4) )/(9*t*u)$
b35:= 16*m^2*z2/(9*t*u)$
c31:= zt/t*c34$
c32:= 2*zt/(s*bet^2)*c36$
c33:= 2*t/s*c34$
c34:= 2*s*( cc6 + s^3 - s^2*t )/(Den*u)$
c35:= zt/(t*bet^2)*c36$
c36:= - 2*s*bet^2*( cc6 - s*u*z2 )/(Den*u)$
d31:= - t*c36$
d32:= - t*c34$

eps2ep2nc:= nc*(con3 + b5(0)*b35 + c1(0)*c31 + c2(0)*c32 + c3(0)*c33
                        + c4(0)*c34 + c5(0)*c35 + c6(0)*c36 + d1(0)*d31 + d2(0)*d32)$


end;


==> nloepf <==
%auto-ignore
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%   notations   %%%%%%%%%%%%%%%%%%%%%
%
%
%    Heavy quark pair production in gluon fusion at next-to-next-to-leading
%       ${\cal O}(\alpha_s^4)$ order: The one-loop squared contributions
%
%
%   This file in REDUCE format gives coefficients in Appendix B
%
%                       Definitions:
%  ep = \epsilon
%  nc = 3, cf = 4/3, da=8 - color factors defined in the paper;
%
%  bet^2=1-4*m^2/s, z2=s+2*t, z2u=s+2*u, zt=2*m^2+t, zu=2*m^2+u;
%  den=D=m^2*s-t*u, tt=t+m^2, uu=u+m^2;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%   Appendix B, Eq.(B1)

noc6:= Den^2*4 - s*bet^2*(8*m^2*s^2 - 8*m^2*t*u - s^3)$
nod3:= 10*m^2*s^2 - 8*m^2*t*u - 3*s*t*u$



b12:= 2*s*( 4*m^2 + z2^2/(s*bet^2) )/(t*u)$
b15:= - b12$
c11:= s*( s^2*bet^2*(8*m^2*s + s^2 + 2*Den) + 4*s^2*Den
                                    - 16*m^2*Den^2/(s*bet^2) - 8*m^4*z2^2 )/(t*u*Den)$
c12:= 2*t*( 2*u*(Den + m^2*s) + s*t^2 + nod3*t/s )/(u*Den)$
c12u:= 2*u*( 2*t*(Den + m^2*s) + s*u^2 + nod3*u/s )/(t*Den)$
c13:= - 2*t*( 2*m^2*s^2 + s*t^2 - nod3*t/s )/(u*Den)$
c13u:= - 2*u*( 2*m^2*s^2 + s*u^2 - nod3*u/s )/(t*Den)$
c14:= s^2*( nod3 + 3*s*Den - s^2*(m^2 - s) )/(t*u*Den)$
c15:= - s*( noc6 + 2*m^2*s*z2^2 )/(t*u*Den)$
c16:= - s*noc6/(t*u*Den)$
d11:= s*t*( z2 + bet^2*(nod3 - s^2*(m^2 - t))/Den )/u$
d11u:= s*u*( z2u + bet^2*(nod3 - s^2*(m^2 - u))/Den )/t$
d12:= s*t*( nod3 + s*Den + s^2*(m^2 - t) )/(u*Den)$
d12u:= s*u*( nod3 + s*Den + s^2*(m^2 - u) )/(t*Den)$
d13:= 2*t*u*nod3/(s*Den)$ 


delep:= ep*(b2(0)*b12 + b5(0)*b15
          + c1(0)*c11 + c2(0)*c12 + c2u(0)*c12u + c3(0)*c13 + c3u(0)*c13u
          + c4(0)*c14 + c5(0)*c15 + c6(0)*c16
          + d1(0)*d11 + d1u(0)*d11u + d2(0)*d12 + d2u(0)*d12u + d3(0)*d13)$

%%%%%%%%%%%   Appendix B, Eq.(B2)

nocc6:= Den*4*t*u + s*bet^2*(18*m^2*s^2 - 16*m^2*t*u - s^3)$
nocd3:= 18*m^2*s^2 - 16*m^2*t*u + s*t*u$


b12:= - 8*m^2*z2^2/(s*t*u*bet^2)$
b15:= - b12$
c11:= - s*( (22*m^2*s^2 - 16*m^2*t*u + s^3)*s*bet^2
                                 + 4*m^2*s*Den - 16*m^2*Den^2/(s*bet^2) )/(t*u*Den)$
c12:= 2*t*( 6*s*Den + 4*m^2*s*z2 + t^2*z2 - nocd3*t/s )/(u*Den)$
c12u:= 2*u*( 6*s*Den + 4*m^2*s*z2u + u^2*z2u - nocd3*u/s )/(t*Den)$
c13:= - 2*t*( nocd3*t/s - s*( 2*m^2*s - 2*s*t - t^2) )/(u*Den)$
c13u:= - 2*u*( nocd3*u/s - s*( 2*m^2*s - 2*s*u - u^2) )/(t*Den)$
c14:= - s^2*( nocd3 + s*Den + s^2*(m^2 + s) )/(t*u*Den)$
c15:= - s*( nocc6 - 2*m^2*s*( Den*4 + z2^2) )/(t*u*Den)$
c16:= - s*nocc6/(t*u*Den)$
d11:= s*t*( Den*2*u - bet^2*(nocd3 - 4*s*t*u - s*t^2) )/(u*Den)$
d11u:= s*u*( Den*2*t - bet^2*(nocd3 - 4*s*t*u - s*u^2) )/(t*Den)$
d12:= - s*t*( nocd3 + s*(2*m^2*s - 2*s*t - t^2) )/(u*Den)$
d12u:= - s*u*( nocd3 + s*(2*m^2*s - 2*s*u - u^2) )/(t*Den)$
d13:= - 2*t*u*nocd3/(s*Den)$

delep2:= ep^2*(b2(0)*b12 + b5(0)*b15
            + c1(0)*c11 + c2(0)*c12 + c2u(0)*c12u + c3(0)*c13 + c3u(0)*c13u
            + c4(0)*c14 + c5(0)*c15 + c6(0)*c16
            + d1(0)*d11 + d1u(0)*d11u + d2(0)*d12 + d2u(0)*d12u + d3(0)*d13)$



%%%%%%%%%%%   Appendix B, Eq.(B3)

colfac:= - (cf + nc/2*t/s)$
tno:=8*z2*
        ( 2*s*(nlf + 1) + b2(0)*3*(8*m^2 + s) + b5(0)*3*s*nlf + c5(0)*18*m^2*s)/(9*s^2)$

nocolep:= - ep*tno*m^2*s/t/u$
nocolep2:= ep^2*tno$

%%nocol:= tno*( - ep*m^2*s/t/u + ep^2 )$


%%%%%%%   Appendix B, Eq.(B4)

sb2:=2*m^2*s - t*z2^2/s/bet^2$
sc2:=t*sc5 - Den*4*m^2*s*u$
sc5:=Den*2*(Den + s*(8*m^2 + t)) + 2*s*t*bet^2*(2*m^2*u - t^2) + s*t^2*z2$
sc6:=Den*(3*s*bet^2 + z2) + bet^2*(6*m^2*s^2 - 8*m^2*t*u + s^2*t)$
%%%%%%%
%%%%%%%   Appendix B, Eq.(B5)

con2:= 8*( 2*m^2*s*bet^2*(4*s*tt^2/t + t*zt - 2*t*u) 
              + Den*(10*m^2*u - 5*s*zt - 2*t^2) - 2*m^2*t*(s^2 + u^2)
              - Den^2*6*t/(s*bet^2) - Den*3*t^2*z2/(s*bet^2) )/(t^2*u*TT)$
b21:= - 8*( Den*(4*m^2*u - s*t) - t^3*(2*s*bet^2 + 3*zt) )/(t^2*u*TT)$
b22:= - 8*sb2/(t*u)$
c22:= 8*sc2/(Den*t*u)$
c25:= 4*s*sc5/(Den*t*u)$
c26:= 4*s*sc6/(Den*u)$
d21:= - t*c26$

cfep:= cf*ep*(con2 + b1(0)*b21 + b2(0)*b22 + c2(0)*c22 + c5(0)*c25 + c6(0)*c26 + d1(0)*d21)$


%%%%%%%   Appendix B, Eq.(B6)

cb2:=2*m^2*u + Den$
cc2:=Den*2*( 4*m^2*s*u - t*Den - s*t*(17*m^2 + 3*t) )
           - 4*s*t^2*bet^2*(2*m^2*u - t^2) + s*t^2*(3*s*zt + 4*m^2*z2)$
cc5:=Den*2*(20*m^2*s - s*t + t^2) + 2*s*t*bet^2*( 4*m^2*u + s*t - 2*t^2) + 5*s*t^2*z2$
cc6:=Den*2*(s*bet^2 - u) + bet^2*(16*m^2*(s^2 - t*u) + s^2*t)$


%%%%%%%   Appendix B, Eq.(B7)

con2:= 8*( Den^2*12*t/(s*bet^2) + Den^2*16*m^2/t
           + Den*4*(2*s*zt - t*u) - Den*t*(14*m^2 + 3*t)/bet^2
           - 2*m^2*(12*m^2*s^2*TT/t + 5*t^3) - 4*m^2*t^2*z2/bet^2 )/(t^2*u*TT)$
b21:= 8*( Den*(4*zt/t^2 + 1/u) + 2*m^2*(t/u - 2) )/TT$
b22:= - 16*z2*cb2/(s*t*u*bet^2)$
c22:= 8*cc2/(Den*t*u)$
c25:= - 4*s*cc5/(Den*t*u)$
c26:= - 4*s*cc6/(Den*u)$
d21:= - t*c26$

cfep2:= cf*ep^2*(con2 + b1(0)*b21 + b2(0)*b22 + c2(0)*c22 + 
                           c5(0)*c25 + c6(0)*c26 + d1(0)*d21)$


%%%%%%%   Appendix B, Eq.(B8)

con2:= 8*( t*z2*(2*m^2 + Den/(s*bet^2))/bet^2 - m^2*(4*s/t*Den - 2*s^2 + t*z2/9) )/(t^2*u)$
b21:= - 8*(3*m^2*s + t*z2)/(t*u)$
b22:= 4*sb2/(t*u)$
b25:= 4*( Den*2*(8*m^2*t + s^2)/(s^2*bet^4) + 4/3*m^2*(s - u) - s*zt/bet^2 )/(t*u)$
c21:= - 2*s*( s^2*bet^4*t/Den + 2*s*bet^2*(2*m^2*z2 - t*u)/Den - 8*m^2*s^2*zt/(t*Den)
            - Den*6/t + 8*t + 2*t*z2/(s*bet^2) - Den*4*zt/(s*t*bet^4) )/u$
c22:= - 4*sc2/(Den*t*u)$
c23:= 2*t/s*c24$
c24:= 2*s*( 8*m^2*u^2/Den + 4*s - s*t*(8*m^2 + s)/Den )/u$
c25:= - 2*s*sc5/(Den*t*u)$
c26:= - 2*s*sc6/(Den*u)$
d21:= - t*c26$
d22:= - t*c24$

ncep:= ep*nc*(con2 + b1(0)*b21 + b2(0)*b22 + b5(0)*b25 + c1(0)*c21 + c2(0)*c22 +
                   + c3(0)*c23 + c4(0)*c24 + c5(0)*c25 + c6(0)*c26 
                   + d1(0)*d21 + d2(0)*d22)$
clear c24;


%%%%%%%   Appendix B, Eq.(B9)

con2:= 8*( 4*m^4*s^2/t - s^2*zt - 10/9*s*t^2 - t^3/3 - 2/9*t^4/s
                       - Den*t*z2/(s*bet^4) + t*(u*z2 + 8*m^2/s*Den)/bet^2 )/(t^2*u)$
b21:= 16*(Den*z2 + t^2*u)/(t^2*u)$
b22:= 8*z2*cb2/(s*t*u*bet^2)$
b25:= - 8*z2*( 4*m^2*Den/(s^2*bet^4) + t*u/s/3 - 2*m^2*u/(s*bet^2) )/(t*u)$
c21:= - 2*s*( 40*m^2*s/t 
                 + (8*m^2*s*u*bet^2 + 20*m^2*s*u + 16*m^2*t^2 - s^2*t)/Den
                 + 2*(2*m^2*s^2/t + 4*m^2*t - s^2)/(s*bet^2)
                 + 8*m^2*Den/(s*t*bet^4) + 4*m^2*(1/s^2 + bet^2/Den)*z2^2/bet^4 )/u$
c22:= - 4*cc2/(Den*t*u)$
c23:= 2*t/s*c24$
c24:= - 2*s*( 20*m^2*s^2 + 4*s*t*u*bet^2 + s*t*z2 )/(Den*u)$
c25:= 2*s*cc5/(Den*t*u)$
c26:= 2*s*cc6/(Den*u)$
d21:= - t*c26$
d22:= - t*c24$

ncep2:= ep^2*nc*(con2 + b1(0)*b21 + b2(0)*b22 + b5(0)*b25 + c1(0)*c21 + c2(0)*c22 +
                         + c3(0)*c23 + c4(0)*c24 + c5(0)*c25 + c6(0)*c26
                         + d1(0)*d21 + d2(0)*d22)$


end;

